DOPING: Generative Data Augmentation for Unsupervised Anomaly Detection with GAN

Recently, the introduction of the generative adversarial network (GAN) and its variants has enabled the generation of realistic synthetic samples, which has been used for enlarging training sets. Previous work primarily focused on data augmentation for semi-supervised and supervised tasks. In this paper, we instead focus on unsupervised anomaly detection and propose a novel generative data augmentation framework optimized for this task. In particular, we propose to oversample infrequent normal samples - normal samples that occur with small probability, e.g., rare normal events. We show that these samples are responsible for false positives in anomaly detection. However, oversampling of infrequent normal samples is challenging for real-world high-dimensional data with multimodal distributions. To address this challenge, we propose to use a GAN variant known as the adversarial autoencoder (AAE) to transform the high-dimensional multimodal data distributions into low-dimensional unimodal latent distributions with well-defined tail probability. Then, we systematically oversample at the `edge' of the latent distributions to increase the density of infrequent normal samples. We show that our oversampling pipeline is a unified one: it is generally applicable to datasets with different complex data distributions. To the best of our knowledge, our method is the first data augmentation technique focused on improving performance in unsupervised anomaly detection. We validate our method by demonstrating consistent improvements across several real-world datasets.

==> sections/analysis_synthetic.tex <==
\section{Analysis of DOPING with Synthetic Datasets}
\label{sec:toy_expt}

In this section, we analyze fundamental components of DOPING  with synthetic datasets. We first demonstrate that the use of the AAE in our framework enables mapping of  diverse data distributions to a consistent latent distribution. This enables a unified analysis, which reveals that there exists a consistent region in the latent space for generating synthetic samples that optimally improve the anomaly detection performance. Most importantly, this sampling method for data augmentation is consistent despite the different data distributions.

\subsection{Dataset and Experimental Design}
\label{sec:toy_expt_setup}

\noindent \textbf{Dataset} We introduce three synthetic datasets that each comprise samples from a normal distribution and an anomalous distribution
(Figure \ref{fig:toy_expt_datasets}).
Each dataset contains 1000 training samples and 1000 test samples, with 95\% of the samples belonging to the normal distribution and 5\% of the samples belonging to the anomalous distribution.

\begin{itemize}
	\item \textbf{Dataset A} The normal distribution is a 2-D Gaussian with mean at origin and standard deviation 10.0 on each dimension, while the anomalous distribution is a 2-D Gaussian with mean [30.0, 0.0] and standard deviation 5.0 on each dimension.
	\item \textbf{Dataset B} A 3-D version of Dataset A with same parameters. 
	%, where the normal distribution is a 3-D Gaussian distribution with mean at the origin and standard deviation 10.0 on each dimension, while the anomalous distribution is a 3-D Gaussian distribution with mean [30.0, 0.0, 0.0] and standard deviation 5.0 on each dimension.
	\item \textbf{Dataset C} The normal distribution follows a ring with radius of mean 30.0 and standard deviation 5.0, while the anomalous distribution is a 2-D Gaussian with mean at origin and standard deviation 5.0 on each dimension. This is meant to be a challenging dataset, with the anomalies surrounded by normal samples, making it more difficult for anomaly detection algorithms to recognize anomalies.
\end{itemize}


\noindent \textbf{Baseline Method} In this experiment, we use the popular iForest anomaly detection algorithm. We use the implementation in version 0.19.1 of the scikit-learn package \cite{scikit-learn} and vary the contamination hyperparameter from 0.01 to 0.69 in increments of 0.04 to generate the receiver operating characteristic (ROC) curve for evaluation.

\noindent \textbf{Implementation} In this section, we first adopt a {\em Labeled AAE} architecture to analyze our method. It is similar to the Unlabeled AAE, with the exception of label information provided to the discriminator network in the form of a one-hot vector. In our case, the label indicates if the sample is normal or anomalous. If the sample is anomalous, we use a ring with radius 100.0 as the prior $p(z)$, by randomly sampling a latent vector with $l^2$-norm of 100.0. If the sample is normal, we follow the prior used in the Unlabeled AAE. All other conditions are the same as described in the Unlabeled AAE.
This Labeled AAE is used {\em only in this analysis} to understand the effectiveness of sampling at different latent regions.  In practice, Unlabeled AAE is used, as will be further discussed.

As mentioned in Section \ref{sec:implementation}, we first use magnitude-based sampling for synthesizing new samples, in order to demonstrate the effects of sampling from different regions in the latent distribution.

We sample latent vectors at different $l^2$-norms from 5.0 to 100.0 at increments of 5.0. At each $l^2$-norm, we decode and add the 100 random samples to the original dataset. Each augmented dataset of 1100 samples is then used to train the anomaly detectors and tested on the test set, to generate the ROC curves. We then measure the area-under-curve (AUC) for each ROC curve and plot the AUC against the $l^2$-norm, as shown in Figure \ref{fig:toy_expt_auc}. We treat predictions of anomalies as positive instances for the calculations of the AUC.

%By training a Labeled AAE on the synthetic dataset, we can impose a latent space where the normal samples are encoded to a Gaussian distribution and the anomalous samples are encoded to a ring with radius 100.0. 

% MAPPING OF DATA SPACES TO LATENT DISTRIBUTIONS

\begin{figure}
	\begin{center}
	\begin{subfigure}[b]{6cm}
	\centering
	\includegraphics[width=6cm]{figures/DatasetA_mapping}
	\caption{}
	\end{subfigure}
    \begin{subfigure}[b]{6cm}
	\centering
	\includegraphics[width=6cm]{figures/DatasetC_mapping}
	\caption{}
	\end{subfigure}
    \end{center}
\caption{Visualization of samples decoded from the latent space of (a) Dataset A and (b) Dataset C. Latent vectors at the boundary of the latent normal distribution (blue) decode to points at the boundary of the normal distribution in the original data space.}
\label{fig:toy_expt}
\end{figure}

\begin{figure*}
\includegraphics[width=18cm]{figures/toy_expt_auc}
\caption{Graphs of AUC against $l^2$-norm/magnitude for the different synthetic datasets, showing a consistent trend.} 
%These are generated by synthesizing 100 samples from rings of different magnitudes or radii in the latent space in Figure \ref{fig:toy_expt} and adding them to the original dataset for training with the iForest detector.}
\label{fig:toy_expt_auc}
\end{figure*}

\subsection{Mapping of Data Spaces to Latent Distributions}
\label{sec:mapping}

%In \cite{makhzani2015}, Makhzani \emph{et al.} demonstrated the mapping of high-dimensional data spaces to low-dimensional latent spaces that could be manipulated to take on certain distributions. Specifically, \cite{makhzani2015} showed the mapping of the MNIST dataset \cite{lecun1998}, Toronto Face dataset \cite{susskind2010} and Street View House Numbers dataset \cite{netzer2011} to various latent distributions including a 2-D Gaussian, a mixture of 10 2-D Gaussians and a swiss roll distribution. In this section, we further demonstrate the ability of AAEs to impose an arbitrary latent distribution.

Figure \ref{fig:toy_expt_datasets} shows 3 different datasets. By training an AAE with the same prior on each of these datasets, we are able to map these datasets to similar latent distributions, in Figure \ref{fig:toy_expt_latent_spaces}. In particular, this happens even for Dataset C, which is particularly challenging since the AAE has to switch the distributions of the normal and anomalous samples.

Furthermore, we are able to systematically sample the latent space to generate corresponding samples in the data space. 
With the use of 2-D Gaussian, which has well-defined tail probability, as the prior, 
we can sample latent vectors of different $l^2$-norms, corresponding to different probabilities or likelihoods. This is akin to sampling latent vectors at rings of different radii, centered on the origin. Since the anomalous latent distribution forms a ring around the normal distribution, as we increase the $l^2$-norm of the sampled latent vectors, the generated samples should intuitively transform from normal to anomalous. Figure \ref{fig:toy_expt} shows the data samples generated by decoding from different rings in the latent space for Datasets A and C. 

% OPTIMAL SAMPLING FROM LATENT SPACE FOR GENERATING SYNTHETIC SAMPLES

\subsection{Optimal Sampling in Latent Space for Generating Synthetic Samples}
\label{sec:optimalregion}

%In Section \ref{sec:problem}, we explained that the task of anomaly detection is often plagued with false positives, since such methods have a high chance of misclassifying infrequent normal samples that are tail ends of the normal distribution. 
In this section, we validate our hypothesis that decoding from the boundary of the normal latent distribution to generate infrequent normal samples provides optimal improvement in anomaly detection performance, when such samples are added to the training set.

%that deliberately increasing the quantity of infrequent normal samples in the training dataset will help density-based methods to better recognize these samples as normal.
%We proceed by decoding 100 samples from rings of different magnitudes in the latent spaces in Figure \ref{fig:toy_expt_latent_spaces} and adding them to the original dataset for training with the iForest detector. We then record the resulting AUC at each magnitude to generate the graphs in Figure \ref{fig:toy_expt_auc}.

All three graphs in Figure \ref{fig:toy_expt_auc} clearly show the same trends, with optimal AUC performance when DOPING with latent vectors of $l^2$-norms in the range of 15.0 to 20.0. With reference to Figure \ref{fig:toy_expt_latent_spaces}, this region corresponds to the boundary of the normal latent distribution, which validates our hypothesis.

The optimal samples for data augmentation is not necessarily intuitive when viewed in the data space. For instance, in Dataset C, it is not immediately clear if the ideal synthetic samples should lie in the inner or outer boundary of the normal distribution. Despite that, Figure \ref{fig:toy_expt_auc} shows that an optimal improvement can be consistently achieved with our method, when decoding from the boundary of the latent distribution. 
Referencing to Figure \ref{fig:toy_expt}  reveals that latent vectors at the boundary of the normal distribution map to data samples on the outer boundary of the normal data. 

Thereafter, as $l^2$-norm increases, the AUC falls to below that of the original dataset, implying that addition of samples in this region actually worsens the performance of the anomaly detectors. In the context of our hypothesis, samples decoded from latent vectors in this region actually corresponds to anomalous samples. By increasing the density of anomalies in the training set, the anomaly detector algorithms are more likely misclassify anomalies as normal, which worsens performance.

\textbf{Unsupervised Data Augmentation} Since samples at the boundary of the normal latent distribution provides the optimal improvement in anomaly detection performance, in practice, the Labeled AAE can be replaced with the unsupervised Unlabeled AAE. We reiterate that the nature of anomaly detection tasks is that "anomalies are 'few and different', which make them more susceptible to isolation than normal points" \cite{liu2008}. With a low contamination rate, an Unlabeled AAE trained on the entire dataset can approximate the normal latent distribution in a Labeled AAE and the contamination due to the 'few and different' anomalies can be neglected. We demonstrate this in the following sections where we only use the Unlabeled AAE.


==> sections/doping.tex <==
\section{DOPING}
\label{sec:doping}

We hereby introduce Doping with Infrequent normal Generator (DOPING), a data augmentation technique for anomaly detection algorithms. In physics, doping is a process whereby a material is introduced into a semiconductor, typically to improve its electrical conductivity. Similarly, our method introduces artificial samples to the original training set, to improve the performance of anomaly detection algorithms. These artificial samples take the form of infrequent normal samples that are synthetically generated with AAEs. 

%In the context of this paper, we define \emph{infrequent normal samples} as samples that are classified as infrequent but exist in the tails of the inherent probability distribution of the normal data. Section \ref{sec:problem} explained that these samples are often misclassified as anomalies, leading to increased false positive rates. Intuitively, DOPING seeks to systematically generate these infrequent normals and add them to the original dataset hence increasing their density, allowing anomaly detectors to better recognize these samples and reducing false positive rates.

%In aiming to systematically generate infrequent normals, we encounter two challenges:
%\begin{enumerate}
%	\item How do we derive the inherent probability distribution of the normal data? 
%	\item How do we generate samples at the tails of this probability distribution? 
%\end{enumerate}	
%It turns out we are able to indirectly solve both problems by using the adversarial aut. 

\noindent \textbf{Adversarial Autoencoders (AAE)~\cite{makhzani2015}.} Consider a dataset with data distribution $p_d(\mathbf{x})$ and an encoding function $q(\mathbf{z}|\mathbf{x})$ from the autoencoder. The aggregated posterior distribution $q(\mathbf{z})$ on the latent vector is then defined as:
\begin{equation*}
q(\mathbf{z}) = \int_\mathbf{x}q(\mathbf{z}|\mathbf{x})p_d(\mathbf{x})\mathrm{d}\mathbf{x}
\end{equation*}
The AAE tries to match $q(\mathbf{z})$ to an arbitrary prior $p(\mathbf{z})$, similar to the variational autoencoder (VAE) \cite{kingma2013}. While the VAE uses the KL-divergence for regularization, the AAE borrows the adversarial concept from the GAN and attaches a discriminator network that discriminates between outputs from the prior $p(\mathbf{z})$ and the encoder $q(\mathbf{z})$. After training, $q(\mathbf{z})$ then matches $p(\mathbf{z})$. Using this mechanism, \cite{makhzani2015} demonstrated several interesting latent spaces including a mixture of 10 2-D Gaussians and a swiss roll distribution.

%Two advantages of the AAE over other GAN variants make it a crucial component of our method.
We specifically choose to adopt AAE over other GAN variants in our framework for the following reasons:
%\begin{description}

\noindent \textbf{Explicit Encoding to Latent Space} While other GAN variants are able to synthesize new samples from a latent space after training, it is non-trivial to encode an arbitrary sample back into the latent space, e.g., requiring iterative estimation \cite{schlegl-ipmi-2017}.
	%a series of backpropagation \cite{schlegl-ipmi-2017}.
	%For example, Schlegl \emph{et al.} \cite{schlegl-ipmi-2017} had to introduce a new mapping schema by defining a loss function for the mapping of new samples to the latent space. The latent vector for a particular sample is then estimated by optimizing the loss function over a series of backpropagation steps. 
In contrast, the AAE already incorporates an autoencoder architecture, which allows explicit decoding from and encoding to the latent space. The encoding network is crucial for our analysis of samples in the latent space, while the decoding network enables generation of synthetic samples from specific regions in the latent space based on our analysis. The encoding and decoding are tightly coupled in  AAE, enabling our analysis outcomes to directly guide sample synthesis.  

\noindent \textbf{Explicit Control of Latent Space} Using the AAE, we are able to  impose a variety of prior distributions on the latent space, similar to the VAE \cite{kingma2013}. However, the VAE requires access to the exact functional form of the prior distribution. In contrast, the adversarial method used by AAE only requires samples from the desired prior, which allows us to impose more complex distributions.
	%The AAE has also been shown to outperform the VAE from the empirical results in \cite{makhzani2015}. 
By imposing the same prior distribution and systematically decoding from this consistent latent space, we have a general method that can be applied to any dataset.
%\end{description}

In our method, we use the AAE to impose a multivariate Gaussian on the latent space of the normal data and treat that as a proxy for the data distribution. 
Our proposed use of multivariate Gaussian as the prior transforms different complex data distributions (e.g. multimodal, skewed) into {\em unimodal ones with well-defined tail probability in the latent space}.
This enables decoding from the edge of the latent Gaussian distribution to generate synthetic samples that are infrequent normals.
As a data augmentation technique, DOPING is used with another anomaly detection algorithm, such as Isolation Forest (iForest) \cite{liu2008}. 
%In Sections \ref{sec:comparison} and \ref{sec:evaluation}, we compare the performance of state-of-the-art anomaly detector algorithms with DOPING and other augmentation techniques, on synthetic and real-world datasets respectively. 
%In the following sections, we will proceed to deconstruct and demonstrate the intuition and components of our method.

%The rest of the paper is organized as follows: Section \ref{sec:implementation} contains implementation details for our method, as well as several variants that we describe and use for analysis. Section \ref{sec:toy_expt} demonstrates the intuition and fundamental components of our method in an experiment with three synthetic datasets. In Section \ref{sec:mnist_expt}, we evaluate the effectiveness of unsupervised DOPING on high-dimensional data. We also compare our method against previous data augmentation methods on various state-of-the-art anomaly detection algorithms. Finally, we evaluate our method on a challenging real-world dataset in Section \ref{sec:landsat_expt}.

% \begin{figure*}
% \includegraphics[width=14cm]{figures/toy_expt_datasets}
% \caption{The three synthetic datasets used in the experiment.}
% \label{fig:toy_expt_datasets}
% \end{figure*}

% \begin{figure*}
% \includegraphics[width=16cm]{figures/toy_expt_latent_spaces}
% \caption{Latent space for each synthetic dataset after training with the AAE. The latent distribution matches a prior distribution of a 2-D Gaussian for the normal samples and approximate a ring distribution for the anomalous samples.}
% \label{fig:toy_expt_latent_spaces}
% \end{figure*}

\begin{figure*}
	\begin{center}
	\begin{subfigure}[b]{13cm}
	\centering
	\includegraphics[width=13cm]{figures/toy_expt_datasets}
	\caption{}
    \label{fig:toy_expt_datasets}
    \end{subfigure}
    %\end{center}
    %\begin{center}
    \begin{subfigure}[b]{16cm}
	\centering
	\includegraphics[width=16cm]{figures/toy_expt_latent_spaces}
	\caption{}
    \label{fig:toy_expt_latent_spaces}
	\end{subfigure}
    \end{center}
\caption{(a) The three synthetic datasets used and (b) the corresponding latent spaces after training with the AAE.}
\end{figure*}

\begin{algorithm}[t]
\caption{InterNN (interpolate with nearest neighbor)}
\label{alg:internn}
\begin{algorithmic}
\REQUIRE $L_{\text{sample}}$: latent vector to interpolate
\STATE Sample $\alpha \sim U(0, 1)$
\STATE $L_{\text{NN}} \leftarrow$ nearest neighbor of $L_{\text{sample}}$ in latent space
\RETURN $\alpha(L_{\text{NN}} - L_{\text{sample}}) + L_{\text{sample}}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{DOPING}
\label{alg:doping}
\begin{algorithmic}
\REQUIRE $K$: no. of samples to synthesize, $D(\cdot)$: decoder and $S_{\text{edge}}$: filtered set of encoded training samples
\STATE Initialize list of synthesized samples $S_{\text{synth}} \leftarrow \text{[]}$
\FOR{$i = 1, 2, ... K$}
\STATE Sample infrequent latent vector $L_{\text{edge}} \in S_{\text{edge}}$
\STATE $L_{\text{new}} \leftarrow \text{\textbf{InterNN}}(L_{\text{edge}})$
\STATE $S_{\text{synth}}$ \textbf{append} $D(L_{\text{new}})$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Design and Implementation}
\label{sec:implementation}

For the following experiments, unless otherwise mentioned, we 
refer to the following design and implementation details.

\noindent \textbf{Train Unlabeled AAE} In DOPING, we first implement the vanilla Unlabeled AAE architecture described in \cite{makhzani2015}, which is detailed in Figure 1 and Appendix A of \cite{makhzani2015}. The encoder, decoder and discriminator each have two layers of 1000 hidden units with ReLU activation function, except for the activation of the last layer of the decoder, which is linear. {\em No labels are used in the training of the Unlabeled AAE}. We use the ADAM optimizer \cite{kingma2014} with a learning rate of $10^{-4}$ for all networks. We use a 2-D Gaussian with mean 0.0 and standard deviation 10.0 on both dimensions as the prior $p(z)$.

%\noindent \textbf{Sample Latent Space.} After training the AAE, we sample random latent vectors at certain $l^2$-norms and decode these latent vectors to generate synthetic samples. As will be discussed, our analysis finds optimal performance when we decode latent vectors at the boundary of the normal latent distribution.

\noindent \textbf{Sample Latent Space} After training the AAE, we selectively sample and decode latent vectors to generate synthetic samples. In the following sections, we will sample latent vectors in two main ways.
\begin{itemize}
	\item \textbf{Magnitude-based} In this case we sample latent vectors from a ring or n-dimensional spherical surface of increasing magnitudes to demonstrate the effects of decoding from different region in the latent distribution. This is used for analysis before we formalize the algorithm.
    \item \textbf{Edge-based} As will be discussed, our analysis finds improved performance when we decode latent vectors at the boundary of the normal latent distribution. Hence, we formalize the DOPING technique as in Algorithm \ref{alg:doping}. We define $S_\text{edge}$ as a filtered subset of the training samples' latent encodings. Implementation-wise, $S_\text{edge}$ is obtained as follows. We first calculate the magnitude of each encoded latent vector as measured from the latent mean. We then discard vectors with magnitudes larger than 3 standard deviations, which we treat as outliers. From the remaining latent vectors, we discard vectors with magnitudes below the 90th percentile. This leaves us with vectors that are at the edge of the latent distribution, not including the outliers, which we define as $S_\text{edge}$. 
\end{itemize}
For Sections \ref{sec:toy_expt} and \ref{sec:mnist_expt}, we first use magnitude-based sampling to analyze effects of sampling from different regions in the latent distribution. The second half of Section \ref{sec:mnist_expt} and Section \ref{sec:landsat_expt} then show the results of using edge-based sampling and compare it against other data augmentation methods.

\noindent \textbf{Train Anomaly Detector with Augmented Data} The synthetic samples are added to the original dataset and the augmented dataset is used to train the anomaly detector algorithm.

In the following sections, we analyze and validate our method with several synthetic datasets, and on an MNIST dataset. Finally, we further evaluate our method on several real-world datasets.

==> sections/introduction.tex <==
\section{Introduction}

One of the key challenges of anomaly detection systems is the pervasiveness of false positives~\cite{chandola2009anomaly}. This is especially true when high true positive rate or recall is required, such as in malware detection, where it is preferable to raise a false alarm rather than let slip an undetected virus.  
High false positive rates can be due to the difficulty in defining a distribution which contains all of the normal data. 
In particular, {\em infrequent normal samples}, defined here as normal samples that occur with very small probability, occur rarely in the training dataset and are poorly characterized in many density-based anomaly detectors \cite{breunig2000, liu2008}. 
In addition, the boundary between normal and anomalous data is typically imprecise, resulting in misclassification of samples close to the boundary \cite{chandola2009anomaly}.

Advancements in deep learning \cite{bengio2009learning, lecun2015deep} have introduced various methods that significantly improve anomaly detection performance \cite{erfani2016high, xu2015learning}. More recently, data augmentation \cite{van2001art} has been used for enlarging the dataset in supervised classification and has shown improved classification performance \cite{perez2017effectiveness, wong2016}. The recent introduction of generative adversarial networks (GANs) \cite{goodfellow2014} also provides a new technique for high-quality data augmentation. 

However, data augmentation has not been explored widely in unsupervised tasks and anomaly detection, likely due to the difficulty of applying data augmentation to such tasks. In supervised classification, data augmentation is primarily used to enlarge a dataset or a specific class in an imbalanced dataset.
But in unsupervised anomaly detection, it is not clear if more normal or anomalous data should be synthesized to improve anomaly detection performance. Specifically, the effectiveness of different types of synthesized samples for anomaly detection has not been systematically studied. As different datasets have different data distributions, it can be challenging to find a general method to create synthetic samples that are effective for anomaly detection.
Furthermore, it is difficult to generate only normal or only anomalous samples in an unsupervised manner without labels. 

In this paper, we propose a data augmentation method targeted at unsupervised anomaly detection, which we coin DOPING. 
Using the adversarial autoencoder (AAE) \cite{makhzani2015}, a GAN variant,
we demonstrate that it is possible to analyze diverse datasets with complicated distributions
in a unified and systematic manner {\em in the latent space}.
Based on the analysis, we propose to strategically 
decode from the latent distribution at specific regions to synthesize samples for augmenting the original dataset. 
In particular, the DOPING technique differs from previous works where GAN architectures were used in anomaly detection:
\begin{itemize}
	\item It is an unsupervised technique that does not require any normal or anomalous labels. Our proposed method trains the AAE on the entire dataset without labels and utilize general knowledge of the latent distribution to generate desired samples. 
	\item Rather than an independent anomaly detection technique, DOPING is a form of unsupervised data augmentation. This makes it complimentary with any anomaly detection algorithm, by augmenting the dataset before training. We demonstrate empirically that using DOPING can help to improve F1 and AUC performance for various anomaly detection tasks.
	\item DOPING differs from previous data augmentation methods, in that it uses a systematic sampling strategy that has been validated in our analysis to be effective for anomaly detection. In contrast, previous methods mainly focused on generating arbitrary artificial samples in a minority class.
\end{itemize}

In this paper, we analyze our method and show that it can be used in an unsupervised setting and is generalizable to different datasets and anomaly detectors. We also compare it to other data augmentation techniques and validate our method on high-dimensional and challenging real-world datasets.

==> sections/motivation.tex <==
\section{Motivation}
\label{sec:problem}

\textbf{Anomaly Detection.} Traditional anomaly detection can be characterized as a typically unsupervised binary classification task with imbalanced data, where the number of normal instances far outweigh the number of anomalous instances. As defined by Hawkins \cite{hawkins1980}: "An outlier is an observation that deviates so much from other observations as to arouse suspicion that it was generated by a different mechanism." Many anomaly detection algorithms take advantage of anomalies being rarer, sparser and of lower density as compared to their normal counterparts. For instance, the Local Outlier Factor (LOF) algorithm "is loosely related to density-based clustering" \cite{breunig2000}, whereas the Isolation Forest (iForest) algorithm is based on the notion that "anomalies are `few and different', which make them more susceptible to isolation than normal points" \cite{liu2008}.

\begin{figure}
\includegraphics[width=8cm]{figures/toy_expt_iforest_fp}
\caption{Isolation Forest predictions on Dataset A in the experiment described in Section \ref{sec:expt_setup}. Points predicted as normal and anomalous are in black and red respectively, while misclassified points are shown as `x', where \emph{false positives} are defined as normal instances that are misclassified as anomalies.}
\label{fig:toy_expt_fp}
\end{figure}

\noindent \textbf{High False Positive Rates.} On the other hand, it has been mentioned in anomaly detection literature that "anomalous points should not just be points in the tails of the `normal' distribution" \cite{emmott2013}. Rather, "anomalous data points should also be from a real-world process that is semantically distinct from the process generating the normal points". Taking this into consideration, many algorithms often misclassify "points in the tails of the `normal' distribution" as anomalies since they appear less frequently and are less dense compared to more common normal points. Misclassifying infrequent normal samples as anomalies then leads directly to increased false positives, where \emph{false positives} are defined as normal instances that are misclassified as anomalies.
For example, Figure \ref{fig:toy_expt_fp} shows an experiment on Dataset A detailed in Section \ref{sec:expt_setup} where the iForest algorithm classifies samples at the edge of a normal distribution as anomalous. 
